A Wave Packet Approach to Interacting Fermions

In this thesis, we study the breakdown of the Fermi liquid state in cuprate superconductors using the renormalization group (RG). We seek to extend earlier work on the crossover from the Fermi liquid state to the pseudo gap phase based on RG flows in the so-called saddle point regime. Progress in the derivation of effective models for the conjectured spin liquid state has been hindered, by the difficulties involved in solving the strong coupling low energy Hamiltonian. We tackle the problem by introducing an orthogonal wave packet basis, the so-called Wilson-Wannier (WW) basis, that can be used to interpolate between the momentum space and the real space descriptions. We show how to combine the WW basis with the RG, such that the RG is used to eliminate high-energy degrees of freedom, and the remaining strongly correlated system is solved approximately in the WW basis. We exemplify the approach for different one-dimensional model systems, and find good qualitative agreement with exact solutions even for very simple approximations. Finally, we reinvestigate the saddle point regime of the two-dimensional Hubbard model. We show that the anti-nodal states are driven to an insulating spin-liquid state with strong singlet pairing correlations, thus corroborating earlier conjectures.

==> chapters/appendices/operator_trafo.tex <==
\chapter{Details for the transformation of operators in one dimension}
\label{app:operator_trafo}

\section{Kinetic energy}
\noindent
In this section we discuss the WW representation of the kinetic energy operator
\begin{equation}
\ham{kin} = \sum_p \epsilon(p) c^\dagger_p\, c^\pdag_p,
\end{equation}
where we assume $\epsilon_p = -2t\cos p$ in the following (more general forms of the dispersion can be dealt with in the same manner, however). $t$ is the hopping rate for nearest neighbor hopping, the bandwidth is $W=4t$.  
\noindent
The wave packet transform of $\epsilon(p)$ by $\bar{T}(m\alpha k,m'\alpha'k')$. We define
\begin{equation}
q_\pm = \frac{\pi}{2M} \left(\alpha k - \alpha'k'\right),
\end{equation}
where $q_{+}$ is the average of the momenta of the two wave packets and $2q_{-}$ is their difference.
From (\ref{eq:O_wave_packet_transform}) we obtain
\begin{eqnarray}
\bar{T}\left(m\alpha k,m'\alpha'k'\right) &=& -2t \sum_{p} \epsilon\left(p+q_{+} \right) \, e^{-iM p\left(m - m' \right)} \, e^{-iM q_{-} \left(m+m'\right)} \,\tilde{g}\left(p+q_{-}\right)\tilde{g}\left(p-q_{-}\right)
\label{eq:T_wave_packet}
\end{eqnarray}
From the momentum space localization of $\tilde{g}(p)$ it follows that for $\left|\alpha k-\alpha'k'\right| > 1$, the RHS of (\ref{eq:T_wave_packet}) vanishes.

\section{Interaction}

==> chapters/appendices/wwtrafo2d.tex <==
\chapter{Transformation of interactions to WW basis in two dimensions}
\section{Saddle points}
\label{sec:sp_transformation_4M}

\noindent
We derive the approximate transformation from momentum space to the truncated WW basis including states at the saddle points only. The derivation is in one dimension for sake of simplicity, but the generalization to higher dimensions is trivial. The momentum space interactions are known on a discrete grid only, which we take to be oversampled by a factor of two, i.e. $N = 4M$, where $N = \frac{2\pi}{\Delta p}$ is related to the Brillouin zone discretization $\Delta p$. Momentum conservation ensures that the WW momentum $k$ is conserved for the truncated expansion. Hence it is sufficient to treat the couplings $g_1,\ldots,g_4$ separately, and the calculation can be based on the window function
\begin{equation}
g_{2m}(j) \equiv g_{2m, 0}(j)
\end{equation}
and its Fourier transform $\tilde{g}_{2m}(p)$. Since $N=4M$, the possible values of $m$ are $m=0,1$. Relatedly, the allowed values for $p$ are $p = -1, 0, 1$, where we have scaled out a factor of $\frac{2\pi}{N}$ for later convenience. The unshifted window function in momentum space is given by
\begin{equation}
\tilde{g}(p) = \left\{\begin{array}{cc} \frac{1}{\sqrt{2}} & p = 0 \\ \frac{1}{2} & \left| p\right| = 1 \end{array}\right. .
\end{equation}
Applying a shift $2m$ in real space leads to
\begin{eqnarray}
\tilde{g}_{2m}(p) &=& \frac{1}{\sqrt{N}} \sum_j \, e^{-\frac{2\pi}{N} p j} \, g\left(j - 2 M m\right) \nonumber \\
&=& \frac{1}{\sqrt{N}}\sum_j e^{-i\frac{4\pi M}{N} p m} e^{-i\frac{2\pi}{N} p j} g\left(j\right) \nonumber \\
&=& \left(-1\right)^{ p m} \tilde{g}(p),
\end{eqnarray}
where the last line follows from $N=4M$. The transformed interaction is then given by
\begin{equation}
U_{2m_1,\ldots,2 m_4} = \frac{1}{2M}\;\frac{1}{2}\sum_{p_1\cdots p_4} \left(-1\right)^{\sum_{i=1}^4 m_i p_i} \, \left[\prod_{i=1}^4 \tilde{g}\left(p_i\right)\right] \,\delta_{p_1+p_2,p_3+p_4} U\left(p_1,p_2,p_3\right),
\end{equation}
where $U\left(p_1,p_2,p_3\right)$ is the renormalized momentum space interaction. The generalization to the two-dimensional saddle point system is 
\begin{eqnarray}
U^{a_1\cdots a_4}_{2\mathbf{m}_1,\ldots,2\mathbf{m}_4} &=& \frac{1}{\left(2M\right)^2}\;\frac{1}{4} \sum_{\mathbf{p}_1\cdots \mathbf{p}_4} \left(-1\right)^{\sum_{i=1}^4 \mathbf{m}_i\cdot \mathbf{p}_i} \left[\prod_{i=1}^4\tilde{G}\left(\mathbf{p}_{i}\right)\right]\, \delta_{\mathbf{p}_1 + \mathbf{p}_2,\mathbf{p}_3+\mathbf{p}_4} \nonumber \\&&\;\times \;U\left(\mathbf{p}^{(a_1)}+\mathbf{p}_1,\mathbf{p}^{(a_2)}+\mathbf{p}_2,\mathbf{p}^{(a_3)}+\mathbf{p}_3\right).
\label{eq:sp_transformation_4M}
\end{eqnarray}
Note that for $\mathbf{p}_i=0$ all momenta lie at one of the saddle points. In order to use the interaction for a larger lattice, the periodic boundary conditions have to be taken into account, and all non-local interactions have to be divided by the number of bonds connecting the sites. Hence nearest neighbor interactions have to be multiplied by $\frac{1}{2}$, and next-to-nearest neighbor interactions by $\frac{1}{4}$.

\section{Other states on the umklapp surface}
\label{sec:gen_transformation_4M}

\noindent
The formula for the transformation of interactions for states other than the saddle point states is different because $k_i \neq 0,M$, so that the WW basis states are given by
\begin{equation}
\Psi_{\mathbf{m},\mathbf{k}}\left(\mathbf{j}\right) = \frac{1}{2} \sum_{\al} e^{-i\al\cdot\Phi_{\mathbf{m}+\mathbf{k}}} G_{\mathbf{m}, A_{\al}\mathbf{k}}\left(\mathbf{j}\right),
\end{equation}
where 
\begin{equation}
A_{\al} = \left(\begin{array}{cc} \alpha_1 & 0 \\ 0 & \alpha_2 \end{array}\right).
\end{equation}

\noindent

\begin{eqnarray}
U_{\mathbf{m}_1\cdots \mathbf{m}_4} &=& \frac{1}{16} \sum_{\al_1\cdots \al_4} e^{-i\left(\al_1\cdot \Phi_{\mathbf{m}_1} + \al_2\cdot \Phi_{\mathbf{m_2}} -\al_3\cdot \Phi_{\mathbf{m}_3} - \al_4\cdot \Phi_{\mathbf{m_4}}\right)} \delta_{\al_1+\al_2,\al_3+\al_4} \, \nonumber \\&& \times \, \frac{1}{N^2}\sum_{\mathbf{p}_1\cdots \mathbf{p}_4} \, e^{-i M\left(\mathbf{m}_1\cdot \mathbf{p}_1 + \mathbf{m}_2\cdot \mathbf{p}_2 - \mathbf{m}_3\cdot \mathbf{p}_3 - \mathbf{m}_4\cdot \mathbf{p}_4\right)} \delta_{\mathbf{p}_1+\mathbf{p}_2,\mathbf{p}_3+\mathbf{p}_4} \nonumber \\ && \times \;U\left(\mathbf{p}^{(\al_1)}+\mathbf{p}_1,\mathbf{p}^{(\al_2)}+\mathbf{p}_2,\mathbf{p}^{(\al_3)}+\mathbf{p}_3\right) \; \prod_{i=1}^4 \tilde{G}\left(\mathbf{p}_i\right).
\end{eqnarray}


==> chapters/ladders/ladders.tex <==
\chapter{Hubbard ladder at half-filling}

\noindent
In this section we discuss the low energy behavior of the SO(5) symmetric Hubbard ladder at half-filling. The renormalization group flow for the Hubbard ladder at half-filling has been derived by Lin and Balents \cite{linbalents}. There it was also shown that the system generically flows to strong coupling, and that the fixed point displays an enhanced SO(8) symmetry. When the high-energy Hamiltonian is SO(5) symmetric, the sytem retains this symmetry, and for repulsive interactions the symmetry is realized by the five fermion bilinears
\begin{eqnarray}
\tilde{\Delta}^x &=& \frac{1}{2}\sigma^z_{\alpha \beta}\,\epsilon_{ab}  \left( R^\pdag_{\alpha a} \, L^\pdag_{\beta b} + R^\dagger_{\alpha b} \,L^\dagger_{\beta a}\right) \nonumber \\
\tilde{\Delta}^y &=& \frac{i}{2}  \sigma^z_{\alpha \beta} \,\epsilon_{ab}\left( R^\pdag_{\alpha a} \, L^\pdag_{\beta b} - R^\dagger_{\alpha b} \, L^\dagger_{\beta a}\right) \nonumber \\
\tilde{s}^i &=& \sigma^x_{\alpha\beta}\,\sigma^i_{ab} \left( R^\dagger_{\alpha a} \, L^\pdag_{\beta b} + L^\dagger_{\alpha a}\, R^\pdag_{\beta b}\right)
\end{eqnarray}
which transform in the vector representation of SO(5). The indices $\alpha, \beta$ refer to the two bands, $a,b$ are spin labels, and we have omitted the position argument. Introducing the vector $\tilde{\mathbf{B}} = \left(\tilde{\Delta}_x, \tilde{\Delta}_y, \tilde{s}^x, \tilde{s}^y, \tilde{s}^z\right)$, the effective interaction at scale $\Lambda$ is given by
\begin{equation}
\ham{int} = u_\Lambda \int dr \, \tilde{\mathbf{B}}(r)\cdot\tilde{\mathbf{B}}(r)
\end{equation}
in the continuum limit. At half-filling the Fermi velocity $v_F$ is the same for both bands. 


\noindent
In order to transform the Hamiltonian into the truncated Wilson basis, we can reuse (\ref{eq:spinhamwilson}) for the spin fluctuations $m^i$ after adding suitable band indices, and (\ref{eq:deltaham}) for the pairing fluctuations $\Delta^i$, because the parity of these bilinears is the same for the ladder and the chain cases. Hence we introduce the spin fluctuation- and pairing operators in the Wilson basis
\begin{eqnarray}
\Delta^x_m &=& \frac{1}{2}\sigma^z_{\alpha\beta} \, \epsilon_{ab} \left(\gamma^\pdag_{\alpha m a} \gamma^\pdag_{\alpha m b} + \gamma^\dagger_{\alpha m b}\,\gamma^\pdag_{\beta m a}\right) \nonumber \\
\Delta^y_m &=& \frac{i}{2}\sigma^z_{\alpha\beta} \, \epsilon_{ab} \left(\gamma^\pdag_{\alpha m a} \gamma^\pdag_{\alpha m b} - \gamma^\dagger_{\alpha m b}\,\gamma^\pdag_{\beta m a}\right) \nonumber \\
s^i_m &=& (-1)^m \sigma^x_{\alpha \beta} \, \sigma^i_{ab}\, \gamma^\dagger_{\alpha m a}\, \gamma^\pdag_{\beta m b}.
\end{eqnarray}
Here $\gamma_{\alpha m a}$ is the annihilator for the Wilson basis state with quantum numbers $(m, k_{F,\alpha})$ for band $\alpha$ and spin $a$. We have introduced the factor $(-1)^m$ in the definition of $s^i_m$ in order to account for the fact that the spin-spin interaction is antiferromagnetic for nearest neighbors. Introducing the vector 
\begin{equation}
\mathbf{B}_m = \left(\Delta^x_m, \Delta^y_m, s^x_m, s^y_m, s^z_m \right),
\end{equation}
the interaction is given by
\begin{equation}
\ham{int} = \frac{u_\Lambda}{2M} \sum_{m m'} V(m-m') \, \mathbf{B}_m \cdot \mathbf{B}_{m'},
\end{equation}
where
\begin{equation}
V(m) = \left\{\begin{array}{lcl} 1 & \text{for} & m=0 \\ \frac{1}{2} & \text{for} & |m| = 1 \\ 0 & \text{for}& |m|>1 \end{array}\right.
\end{equation}


\noindent
The  hopping term is given by $t = \frac{\pi v_F}{M}$ as before.

\noindent
At half-filling the Fermi points are located at $\pm \left(\frac{\pi}{2} + \delta p\right)$ and $\pm \left(\frac{\pi}{2} - \delta p\right)$, where $2\delta p$ is the difference between the Fermi momenta of the two bands. The condition of half-filling implies that there are four fermions per WW unit cell in the states centered around the Fermi points.


\noindent
In order to understand the physics of the model, we again apply the contractor renormalization method. The local Hamiltonian is given by
\begin{equation}
\ham{loc} = \frac{u_\Lambda}{2M} \sum_m \mathbf{B}^\dagger_m\cdot \mathbf{B}^\pdag_m,
\end{equation}
and direct diagonalization shows that there is a non-degenerate groundstate with two electrons per site that form a singlet. The lowest excitation energy is five fold degenerate (two singlet pair states and three triplet spin excitations), and the five states transform in the vector representation of SO(5). Thus we keep the groundstate and the five vector states per site, so that there are six states per site in the projected Hilbert space. We represent the five excited states by a hardcore vector boson $\mathbf{b}_m$.

\noindent
In order to find the effective interactions at the two-site level, we diagonalize a two-site cluster and project onto the tensor product space of low energy states as before. The form of the Hamiltonian is restricted due to the high degree of symmetry of the model. Apart from mass and hopping terms interactions between the bosons as well as creation and annihilation of singlet pairs are generated by the renormalization. We can use the decomposition of the tensor product representation of two vector representations of SO(5) in order two find all possible interaction terms. The decomposition is
\begin{equation}
\mathbf{5}\otimes \mathbf{5} = \mathbf{14}\oplus\mathbf{10}\oplus \mathbf{1},
\end{equation}
i.e. two vector bosons on adjacent sites can be either in the singlet representation $\mathbf{1}$, the antisymmetric tensor representation $\mathbf{10}$, or the symmetric tensor representation $\mathbf{14}$. Hence the general form of the Hamiltonian with two-site interactions is
\begin{eqnarray}
\ham{eff} &=& \mu \sum_{m} \mathbf{b}^\dagger_{m}\cdot \mathbf{b}^\pdag_{m} - t_B \sum_{m} \left(  \mathbf{b}^\dagger_{m}\cdot \mathbf{b}^\pdag_{m+1} + \text{h.c.}\right)
+  \sum_{m} \left(t_S \,S^\pdag_m + t_S^\ast \, S^\dagger_m\right) \nonumber \\
&& + \sum_m \left[ U_S\, S_m^\dagger\,S_m + U_A \,\mathbf{A}^\dagger_m \cdot \mathbf{A}_m + U_T \,\mathbf{T}^\dagger_m \cdot \mathbf{T}^\pdag_m\right], 
\label{eq:so5ham}
\end{eqnarray}
where the operators $S_m$, $\mathbf{A}_m$, and $\mathbf{T}_m$ are annihilators for the pair states at sites $m$ and $m+1$ in the singlet, antisymmetric tensor, and symmetric tensor representations, respectively.

\noindent
We determine numerical values of the various coefficients in (\ref{eq:so5ham}) by applying the CORE algorithm. Since our main interest here is to establish the phase diagram, we focus on the gaps of the vector bosons. At half-filling, the system has SO$(5)$ symmetry, so that all bosons have the same gap. In fig. \ref{fig:ladder_gap_scaling}, we show the finite size scaling of the pair gap for system sizes $L$ (number of WW sites) ranging from $L=4$ to $L=8$. Even though the range of system sizes is small, it is apparent that the gap does not scale to zero as the system size is increased, but instead saturates at a finite value, so that we conclude that the effective model (\ref{eq:so5ham}) is gapped in the thermodynamic limit. The inferred correlation length $\lambda$ of the vector bosons is of order one, indicating that the local groundstate is a reasonable approximation of the renormalized groundstate found using CORE. 	
\begin{figure}
\centering
\includegraphics[width=7cm]{fig/ladder_gap_scaling}
\caption{Finite size scaling of the pair gap (representative for all vector boson gaps) in the Hubbard ladder at half-filling. Gaps are obtained from exact diagonalization of the Hamiltonian (\ref{eq:so5ham}). The system sizes considered are $L=4,6,8$, and we impose periodic boundary conditions. The line is a fit of the function $a \,e^{-L/\lambda} + c$ to the data, where $\lambda$ is the correlation length and $c$ is the estimated gap in the thermodynamic limit. We find $\lambda = 1.1$ from the fit. It can be seen that the pair gap converges to its inferred asymptotic value for $L\rightarrow \infty$ very rapidly, so that we expect the system to be gapped in the thermodynamic limit.}
\label{fig:ladder_gap_scaling}
\end{figure}



\noindent
The behavior of the model at small doping can be inferred from the model as well. The cases of hole- and electron-doping are equivalent by virtue of particle-hole symmetry, so that we only deal with the hole-doped case without loss of generality. Since we know from the local Hamiltonian that the energy of a pair of holes is lower than the energy of two separate holes, our approximate treatment of the fermion excitation via contractor renormalization is still valid. Once hole-pairs are introduced into the system, they can move freely, and the gap in the charge sector vanishes. Moreover, because all doped holes are bound into pairs, the system becomes superfluid with a superfluid weight that is expected to be proportional to the number of doped holes. The interaction terms in (\ref{eq:so5ham}) are not important for the phenomenology as long as the density of hole pairs is small. For larger densities, the model is not valid anymore because it is based on the RG flow at half-filling.

